Automatic Bill of Materials

Ensuring the security of software supply chains requires reliable identification of upstream dependencies. We present the Automatic Bill of Materials, or ABOM, a technique for embedding dependency metadata in binaries at compile time. Rather than relying on developers to explicitly enumerate dependency names and versions, ABOM embeds a hash of each distinct input source code file into the binary emitted by a compiler. Hashes are stored in Compressed Bloom Filters, highly space-efficient probabilistic data structures, which enable querying for the presence of dependencies without the possibility of false negatives. If leveraged across the ecosystem, ABOMs provide a zero-touch, backwards-compatible, drop-in solution for fast supply chain attack detection in real-world, language-independent software.

==> algorithms/index_folding.tex <==
\begin{algorithm}
\caption{Index Folding}
\begin{algorithmic}
\label{alg:index_folding}
\STATE\textbf{Input:} Bloom filter length $m$ (restricted to power of 2), number of indices $k$, hash value $H$ of length $h$
\STATE\textbf{Output:} $k$ indices of $0\leq{}i<m$
\STATE
\STATE $b \gets \log_2(m) \times k$
\WHILE[Expand Hash]{$h < b$}
    \STATE $H \gets$ concat($H$, SHA3\_256($H$))
\ENDWHILE
\STATE
\STATE $K \gets [\ ]$
\FOR[Compress Hash]{$i \gets 0$ \textbf{to} $k$}
    \STATE $x \gets 0$
    \FOR{$j \gets 0$ \textbf{to} $\lfloor h / b\rfloor$}
        \STATE $x \gets x\ \oplus\ H_{i\times k + j}$
    \ENDFOR
    \STATE append($K$, $x$)
\ENDFOR
\FOR{$i \gets 0$ \textbf{to} $h\mod{b}$}
    \STATE $K_k \gets K_k\ \oplus\ H_{h-i}$
\ENDFOR
\STATE
\RETURN $K$\COMMENT{Return Indices}
\end{algorithmic}
\end{algorithm}
